Large-scale Monte Carlo/Molecular Dynamics simulations with Atomic Cluster Expansion potentials in LAMMPS

Monte Carlo/molecular dynamics (MCMD) simulations are widely used to study the properties of materials at the mesoscale. Simulations with hundreds of thousands of atoms usually rely on empirical potentials because MCMD with machine-learning interatomic potentials is impractical at this scale in existing implementations. Here, we introduce a hybrid MPI/OpenMP scheme for MCMD with Atomic Cluster Expansion (ACE) potentials in LAMMPS. Monte Carlo moves are evaluated from local energy changes and carried out in parallel over MPI ranks, while molecular dynamics is parallelized over OpenMP threads. At a fixed number of CPUs, the wall time of the Monte Carlo moves decreases by a factor equal to the number of MPI ranks. Larger simulation cells also reduce the statistical errors of free energy calculations because thermal fluctuations decrease with system size. We demonstrate the scheme by calculating free energies of the HCP and BCC phases in the strongly anharmonic Hf--Ti system and by simulating zirconium segregation in a nanocrystalline copper sample of 670,000 atoms. For Cu--Zr, an ACE potential and an empirical potential predict similar grain boundary compositions but different amounts of zirconium dissolved in the grains. The scheme makes MCMD simulations with machine-learning interatomic potentials practical at the length scales of microstructure.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
